Known Boundary Emulation of Complex Computer Models

Computer models are now widely used across a range of scientific disciplines to describe various complex physical systems, however to perform full uncertainty quantification we often need to employ emulators. An emulator is a fast statistical construct that mimics the complex computer model, and greatly aids the vastly more computationally intensive uncertainty quantification calculations that a serious scientific analysis often requires. In some cases, the complex model can be solved far more efficiently for certain parameter settings, leading to boundaries or hyperplanes in the input parameter space where the model is essentially known. We show that for a large class of Gaussian process style emulators, multiple boundaries can be formally incorporated into the emulation process, by Bayesian updating of the emulators with respect to the boundaries, for trivial computational cost. The resulting updated emulator equations are given analytically. This leads to emulators that possess increased accuracy across large portions of the input parameter space. We also describe how a user can incorporate such boundaries within standard black box GP emulation packages that are currently available, without altering the core code. Appropriate designs of model runs in the presence of known boundaries are then analysed, with two kinds of general purpose designs proposed. We then apply the improved emulation and design methodology to an important systems biology model of hormonal crosstalk in Arabidopsis Thaliana.

==> Known Boundary Emulation Paper 1 JUQ version 3 May 2019/KB_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Known Boundary Emulation of Complex Computer Models}{I. Vernon, S. Jackson, and J. A. Cumming}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Known Boundary Emulation of Complex Computer Models
%\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}
}

% Authors: full names plus addresses.
\author{Ian Vernon\thanks{Department of Mathematical Sciences, Durham University, Stockton Road, DH1 3LE Durham, UK 
  (\email{i.r.vernon@durham.ac.uk}, \email{samuel.jackson@durham.ac.uk}, \email{j.a.cumming@durham.ac.uk})}
\and Samuel E. Jackson\footnotemark[1] 
\and Jonathan A. Cumming\footnotemark[1]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


\usepackage{lscape,epsfig,amsmath,setspace}
\usepackage{xypic}

%\usepackage{natbib}
\usepackage{acronym}
%\usepackage{enumerate}
\usepackage{color}
\usepackage{multirow}
\usepackage{subcaption}

\newcommand{\BE}[2]{\text{E}_{#1}{[#2]}}
\newcommand{\BV}[2]{\text{Var}_{#1}{[#2]}}
\newcommand{\BC}[3]{\text{Cov}_{#1}{[#2},{#3}]}


\usepackage{amsmath,amsfonts,amssymb}
\usepackage[all]{xy}
\usepackage{psfrag}


\usepackage{fullpage} 
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{psfrag}
\usepackage{epsfig}
\usepackage[all]{xy}
\usepackage[linewidth=1pt]{mdframed}


\newcommand{\e}[1]{\ensuremath{{\rm E}\left[#1\right]}}
\newcommand{\ed}[2]{\ensuremath{{\rm E}_{#1}\left[#2\right]}}
\newcommand{\var}[1]{\ensuremath{{\rm Var}\left[#1\right]}}
\newcommand{\rvar}[1]{\ensuremath{{\rm RVar}(#1)}}
\newcommand{\vard}[2]{\ensuremath{{\rm Var}_{#1}\left[#2\right]}}
\newcommand{\rvard}[2]{\ensuremath{{\rm RVar}_{#1}(#2)}}
\newcommand{\corr}[2]{\ensuremath{{\rm Corr}\left(#1,#2\right)}}
\newcommand{\corrd}[3]{\ensuremath{{\rm Corr}_{#1}\left(#2,#3\right)}}
\newcommand{\cov}[2]{\ensuremath{{\rm Cov}\left[#1,#2\right]}}
\newcommand{\covd}[3]{\ensuremath{{\rm Cov}_{#1}\left[#2,#3\right]}}
\newcommand{\covb}[2]{\ensuremath{{\rm Cov}[#1,#2]}}


\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bn}{\begin{enumerate}}
\newcommand{\en}{\end{enumerate}}
\newcommand{\bfi}{\begin{figure}}
\newcommand{\efi}{\end{figure}}

\newcommand{\cm}[1]{\ensuremath{ { #1 }}}

\newcommand{\mx}{\mathcal{X}}
\newcommand{\mk}{\mathcal{K}}
\newcommand{\ml}{\mathcal{L}}

\newcommand{\qq}{\quad \quad}

\newcommand{\ian}[1]{\textcolor{red}{[IRV: #1]}}% IRV comments/changes		
\newcommand{\sam}[1]{\textcolor{blue}{SEJ: #1]}}% IRV comments/changes		
\newcommand{\jdog}[1]{\textcolor{green}{[JAC: #1]}}% IRV comments/changes		

\newcommand{\todo}[1]{\textcolor{red}{#1}}



% for changing the margin 
\newenvironment{changemargin}[2]{%
\begin{list}{}{%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{#1}%
\setlength{\rightmargin}{#2}%
\setlength{\listparindent}{\parindent}%
\setlength{\itemindent}{\parindent}%
\setlength{\parsep}{\parskip}%
}%
\item[]}{\end{list}}


\evensidemargin -0.3cm
\oddsidemargin  -0.3cm
\topmargin 0.3cm
\textwidth 17.2cm
\textheight 24.cm



%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

